Can Code-Switched Texts Activate a Knowledge Switch in LLMs? A Case Study on English-Korean Code-Switching

Recent large language models (LLMs) demonstrate multilingual abilities, yet they are English-centric due to dominance of English in training corpora. The limited resource for low-resource languages remains a crucial challenge. Code-switching (CS), a phenomenon where multilingual speakers alternate between languages in a discourse, can convey subtle cultural and linguistic nuances that can be otherwise lost in translation and elicits language-specific knowledge in human communications. In light of this, we investigate whether code-switching can activate, or identify and leverage knowledge for reasoning when LLMs solve low-resource language tasks. To facilitate the research, we first present EnKoQA, a synthetic English-Korean CS question-answering dataset. We provide comprehensive analysis on a variety of multilingual LLMs by subdividing activation process into knowledge identification and knowledge leveraging. Our results demonstrate that compared to English text, CS can faithfully activate knowledge inside LLMs especially on language-specific domains, suggesting the potential of code-switching on low-resource language tasks.

==> figure_latex/dataset_plain.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\textwidth]{figure_file/dataset_plain.png}
    
    \caption{Experimental results of \magenta{CS} and \teal{EN}.}
    
    \label{fig:dataset_plain} 
    
\end{figure*} 

==> figure_latex/kor_en_cs.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figure_file/ko_en_cs.pdf}
    
    \caption{Correlation between QA accuracy of models in Korean, English, and CS. \textcolor{red}{Red} marker indicates the the model of which the accuracy is higher in CS than in English, and vice versa for \textcolor{blue}{blue} marker. The size of the marker is proportional to the performance of the model. }
    
    \label{fig:ko_en_cs} 
    
\end{figure} 

==> figure_latex/task_desc.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figure_file/task_desc.pdf}
    
    \caption{Illustration of Knowledge Identification (\textit{top}), and Knowledge Leveraging (\textit{bottom}).}
    
    \label{fig:task_desc} 
    
\end{figure} 

==> tables/kor_0518.tex <==



\begin{table*}[!t]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{lc cccccccccc}
\toprule 
  Model & &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  \textbf{Total} \\
\midrule

\multirow{3}{*}{\textbf{GPT-4o}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{91.53} & \cellgray \textbf{\green{78.41}} & \cellgray \textbf{69.04} & \cellgray \textbf{\green{74.79}} & \cellgray \textbf{55.86} & \cellgray \textbf{\green{90.48}} & \cellgray \textbf{\green{95.12}} & \cellgray \textbf{63.7} & \cellgray \textbf{\green{85.14}} & \cellgray \textbf{78.23} \\
& EN & 89.83 & 75.00 & 66.19 & 61.97 & 52.64 & 84.52 & \textbf{\green{95.12}} & 60.4 & 74.32 & 73.33 \\
& KO & 89.83 & 71.59 & 60.14 & 63.03 & 48.74 & 85.71 & 92.68 & 56.44 & 75.23 & 71.49 \\
\midrule

\multirow{3}{*}{\textbf{GPT-3.5}} &
% \rowcolor{defaultcolor} 
\cellgray CS & \cellgray \textbf{71.19} & \cellgray 47.73 & \cellgray 44.48 & \cellgray 32.91 & \cellgray 35.40 & \cellgray \textbf{70.24} & \cellgray \textbf{80.49} & \cellgray 49.17 & \cellgray 57.21 & \cellgray \textbf{54.31} \\
& EN & \textbf{71.19} & \textbf{48.86} & \textbf{45.55} & \textbf{36.32} & \textbf{36.55} & 66.67 & 63.41 & \textbf{52.64} & \textbf{62.61} & 53.76 \\
& KO & 62.71 & 26.7 & 31.67 & 26.71 & 24.83 & 48.81 & 58.54 & 37.79 & 49.55 & 40.81 \\
\midrule

\multirow{3}{*}{\textbf{Claude 3.5}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{\green{93.22}} & \cellgray \textbf{72.16} & \cellgray \textbf{\green{72.95}} & \cellgray \textbf{73.08} & \cellgray \textbf{\green{62.53}} & \cellgray \textbf{86.90} & \cellgray \textbf{\green{95.12}} & \cellgray \textbf{\green{67.66}} & \cellgray \textbf{84.23} & \cellgray \textbf{78.65}
\\
& EN & 89.83 & 71.59 & 67.97 & 61.54 & 55.63 & 85.71 & 92.68 & 63.20 & 75.23 & 73.71 \\
& KO & 64.41 & 47.73 & 54.09 & 54.49 & 45.52 & 69.05 & 82.93 & 52.31 & 61.71 & 59.14 \\
\midrule

\multirow{3}{*}{\textbf{Solar}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{83.05} & \cellgray \textbf{55.11} & \cellgray \textbf{54.09} & \cellgray \textbf{63.46} & \cellgray \textbf{42.76} & \cellgray \textbf{80.95} & \cellgray \textbf{85.37} & \cellgray \textbf{54.29} & \cellgray \textbf{75.23} & \cellgray \textbf{66.03}
\\
& EN & 74.58 & 46.02 & 49.47 & 39.53 & \textbf{42.76} & 77.38 & 65.85 & 51.16 & 62.61 & 56.60 \\
& KO & 81.36 & 50.57 & 56.94 & 58.12 & 46.44 & 82.14 & 78.05 & 54.95 & 70.27 & 64.31 \\
\midrule

\multirow{3}{*}{\textbf{Llama3 70B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray 79.66 & \cellgray 51.70 & \cellgray \textbf{50.53} & \cellgray \textbf{49.36} & \cellgray 44.14 & \cellgray \textbf{80.95} & \cellgray \textbf{75.61} & \cellgray \textbf{57.43} & \cellgray 65.77 & \cellgray \textbf{61.68}
\\
& EN & \textbf{83.05} & \textbf{57.39} & \textbf{50.53} & 45.94 & \textbf{45.75} & 73.81 & 73.17 & 53.30 & \textbf{66.67} & 61.07 \\
& KO & 76.27 & 50.57 & 46.98 & 43.8 & 38.16 & 70.24 & 82.93 & 51.49 & 61.26 & 57.97 \\
\midrule

\multirow{3}{*}{\textbf{Llama3 8B}} &
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{69.49} & \cellgray \textbf{40.34} & \cellgray 36.30 & \cellgray 35.68 & \cellgray \textbf{35.63} & \cellgray \textbf{75.00} & \cellgray \textbf{73.17} & \cellgray 45.05 & \cellgray \textbf{54.05} & \cellgray \textbf{51.63}
\\
& EN & 64.41 & 39.77 & 37.72 & \textbf{37.39} & 32.64 & 67.86 & 63.41 & \textbf{45.21} & 53.6 & 49.11 \\
& KO & 61.02 & 38.07 & 38.79 & 32.48 & 33.33 & 65.48 & 65.85 & 43.73 & 50.9 & 47.74 \\
\midrule

\multirow{3}{*}{\textbf{Gemma2 27B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray 79.66 & \cellgray 46.02 & \cellgray \textbf{48.75} & \cellgray \textbf{41.03} & \cellgray \textbf{45.29} & \cellgray \textbf{77.38} & \cellgray \textbf{78.05} & \cellgray 54.79 & \cellgray \textbf{65.32} & \cellgray 59.59
\\
& EN & \textbf{84.75} & \textbf{53.41} & 48.40 & 40.6 & 41.84 & 72.62 & \textbf{78.05} & \textbf{54.95} & 63.96 & \textbf{59.84} \\
& KO & 77.97 & 44.89 & 44.84 & 41.67 & 41.84 & 73.81 & 75.61 & 50.66 & 59.46 & 56.75 \\
\midrule

\multirow{3}{*}{\textbf{Gemma2 9B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{79.66} & \cellgray 42.05 & \cellgray 44.13 & \cellgray \textbf{40.17} & \cellgray 41.15 & \cellgray \textbf{73.81} & \cellgray \textbf{80.49} & \cellgray \textbf{53.30} & \cellgray \textbf{65.77} & \cellgray \textbf{57.84}
\\
& EN & 76.27 & \textbf{46.02} & \textbf{49.47} & 38.46 & \textbf{42.30} & 69.05 & 73.17 & 52.15 & 63.51 & 56.71 \\
& KO & 76.27 & 42.05 & 41.99 & 34.62 & 40.23 & 71.43 & 82.93 & 51.98 & 58.11 & 55.51 \\
\bottomrule
\end{tabular}
}

\caption{QA performances of multilingual LLMs on CS, English, and Korean settings. \textbf{Bold} indicates higher score between CS and English on each model. \green{\textbf{Green}} indicates the highest score from each domain.}
\label{tab:kor_result}
\end{table*}



==> tables/llm_faith.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{lc cccccccccc}
\toprule 
  Model & &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  Average \\
\midrule


\multirow{2}{*}{\textbf{GPT-4o}}
& \cellgray CS & \cellgray 2.575 & \cellgray 2.375 & \cellgray 2.35 & \cellgray 2.025 & \cellgray 2.425 & \cellgray 2.8 & \cellgray 2.925 & \cellgray 2.2 & \cellgray 2.1  \\
& \ EN & \ 2.5 & \ 2.325 & \ 2.325 & \ 2.025 & \ 2.475 & \ 2.775 & \ 2.925 & \ 2.2 & \ 2.2  \\
\midrule
\multirow{2}{*}{\textbf{GPT-3.5}}
& \cellgray CS & \cellgray 2.675 & \cellgray 2.15 & \cellgray 2.55 & \cellgray 1.925 & \cellgray 2.4 & \cellgray 2.65 & \cellgray 2.65 & \cellgray 2.375 & \cellgray 2.275  \\
& \ EN & \ 2.675 & \ 2.15 & \ 2.575 & \ 1.85 & \ 2.4 & \ 2.625 & \ 2.675 & \ 2.325 & \ 2.3  \\
\midrule
\multirow{2}{*}{\textbf{Claude 3.5}}
& \cellgray CS & \cellgray 2.875 & \cellgray 2.3 & \cellgray 2.5 & \cellgray 2.325 & \cellgray 2.6 & \cellgray 2.9 & \cellgray 2.9 & \cellgray 2.425 & \cellgray 2.4  \\
& \ EN & \ 2.925 & \ 2.4 & \ 2.6 & \ 2.3 & \ 2.525 & \ 2.95 & \ 2.875 & \ 2.425 & \ 2.425  \\
\midrule
\multirow{2}{*}{\textbf{Solar}}
& \cellgray CS & \cellgray 2.75 & \cellgray 2.025 & \cellgray 2.5 & \cellgray 1.75 & \cellgray 2.325 & \cellgray 2.625 & \cellgray 2.65 & \cellgray 2.3 & \cellgray 1.8  \\
& \ EN & \ 2.775 & \ 2.025 & \ 2.5 & \ 1.75 & \ 2.275 & \ 2.625 & \ 2.65 & \ 2.35 & \ 1.8  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 70B}}
& \cellgray CS & \cellgray 2.725 & \cellgray 2.225 & \cellgray 2.525 & \cellgray 1.825 & \cellgray 2.2 & \cellgray 2.7 & \cellgray 2.75 & \cellgray 2.425 & \cellgray 1.975  \\
& \ EN & \ 2.65 & \ 2.2 & \ 2.45 & \ 1.85 & \ 2.35 & \ 2.675 & \ 2.75 & \ 2.35 & \ 1.925  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 8B}}
& \cellgray CS & \cellgray 2.55 & \cellgray 2.025 & \cellgray 2.375 & \cellgray 1.55 & \cellgray 2.15 & \cellgray 2.35 & \cellgray 2.525 & \cellgray 1.925 & \cellgray 1.925  \\
& \ EN & \ 2.575 & \ 1.925 & \ 2.325 & \ 1.575 & \ 2.175 & \ 2.325 & \ 2.5 & \ 1.85 & \ 1.925  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 27B}}
& \cellgray CS & \cellgray 2.7 & \cellgray 2.325 & \cellgray 2.475 & \cellgray 1.875 & \cellgray 2.275 & \cellgray 2.4 & \cellgray 2.8 & \cellgray 2.4 & \cellgray 2.075  \\
& \ EN & \ 2.675 & \ 2.325 & \ 2.425 & \ 1.875 & \ 2.275 & \ 2.45 & \ 2.8 & \ 2.4 & \ 2.0  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 9B}}
& \cellgray CS & \cellgray 2.525 & \cellgray 2.2 & \cellgray 2.475 & \cellgray 1.9 & \cellgray 2.225 & \cellgray 2.575 & \cellgray 2.7 & \cellgray 2.325 & \cellgray 2.075  \\
& \ EN & \ 2.575 & \ 2.225 & \ 2.425 & \ 1.875 & \ 2.25 & \ 2.6 & \ 2.7 & \ 2.325 & \ 2.025  \\
\bottomrule








\end{tabular}
}

\caption{LLM Evaluation on Faithfulness.}
\label{tab:llm_faith}

\end{table*}

==> tables/llm_help.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{lc cccccccccc}
\toprule 
  Model & &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  Average \\
\midrule


\multirow{2}{*}{\textbf{GPT-4o}}
& \cellgray CS & \cellgray 2.55 & \cellgray 2.05 & \cellgray 1.95 & \cellgray 1.75 & \cellgray 2.125 & \cellgray 2.65 & \cellgray 2.9 & \cellgray 1.95 & \cellgray 1.925  \\
& \ EN & \ 2.5 & \ 2.1 & \ 1.925 & \ 1.75 & \ 2.125 & \ 2.625 & \ 2.9 & \ 1.925 & \ 1.95  \\
\midrule
\multirow{2}{*}{\textbf{GPT-3.5}}
& \cellgray CS & \cellgray 2.6 & \cellgray 2.05 & \cellgray 2.15 & \cellgray 1.825 & \cellgray 2.175 & \cellgray 2.5 & \cellgray 2.6 & \cellgray 2.15 & \cellgray 2.2  \\
& \ EN & \ 2.65 & \ 2.075 & \ 2.125 & \ 1.775 & \ 2.175 & \ 2.525 & \ 2.625 & \ 2.15 & \ 2.225  \\
\midrule
\multirow{2}{*}{\textbf{Claude 3.5}}
& \cellgray CS & \cellgray 2.825 & \cellgray 1.95 & \cellgray 2.2 & \cellgray 2.025 & \cellgray 2.15 & \cellgray 2.75 & \cellgray 2.9 & \cellgray 2.15 & \cellgray 2.025  \\
& \ EN & \ 2.825 & \ 2.025 & \ 2.2 & \ 1.95 & \ 2.275 & \ 2.75 & \ 2.875 & \ 2.1 & \ 1.975  \\
\midrule
\multirow{2}{*}{\textbf{Solar}}
& \cellgray CS & \cellgray 2.725 & \cellgray 2.0 & \cellgray 2.15 & \cellgray 1.625 & \cellgray 2.1 & \cellgray 2.55 & \cellgray 2.675 & \cellgray 2.075 & \cellgray 1.725  \\
& \ EN & \ 2.75 & \ 1.9 & \ 2.125 & \ 1.575 & \ 2.05 & \ 2.5 & \ 2.7 & \ 2.075 & \ 1.65  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 70B}}
& \cellgray CS & \cellgray 2.65 & \cellgray 1.925 & \cellgray 2.1 & \cellgray 1.675 & \cellgray 2.05 & \cellgray 2.55 & \cellgray 2.725 & \cellgray 2.025 & \cellgray 1.85  \\
& \ EN & \ 2.625 & \ 1.875 & \ 2.15 & \ 1.675 & \ 2.075 & \ 2.575 & \ 2.725 & \ 2.025 & \ 1.825  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 8B}}
& \cellgray CS & \cellgray 2.475 & \cellgray 1.875 & \cellgray 1.9 & \cellgray 1.5 & \cellgray 2.0 & \cellgray 2.2 & \cellgray 2.5 & \cellgray 1.725 & \cellgray 1.725  \\
& \ EN & \ 2.475 & \ 1.875 & \ 1.9 & \ 1.525 & \ 2.0 & \ 2.2 & \ 2.525 & \ 1.775 & \ 1.775  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 27B}}
& \cellgray CS & \cellgray 2.55 & \cellgray 1.725 & \cellgray 2.05 & \cellgray 1.625 & \cellgray 2.0 & \cellgray 2.1 & \cellgray 2.775 & \cellgray 1.925 & \cellgray 1.85  \\
& \ EN & \ 2.475 & \ 1.775 & \ 2.05 & \ 1.625 & \ 2.05 & \ 2.1 & \ 2.775 & \ 1.85 & \ 1.825  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 9B}}
& \cellgray CS & \cellgray 2.225 & \cellgray 1.775 & \cellgray 1.975 & \cellgray 1.65 & \cellgray 1.875 & \cellgray 2.25 & \cellgray 2.675 & \cellgray 1.9 & \cellgray 1.85  \\
& \ EN & \ 2.25 & \ 1.775 & \ 1.95 & \ 1.625 & \ 1.85 & \ 2.275 & \ 2.65 & \ 1.875 & \ 1.775  \\
\bottomrule




\end{tabular}
}

\caption{LLM Evaluation on Helpfulness}
\label{tab:llm_help}

\end{table*}

==> tables/llm_pair.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{lc cccccccccc}
\toprule 
  Model & &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  Average \\
\midrule


\multirow{2}{*}{\textbf{GPT-4o}}
& \cellgray CS & \cellgray 35.0 & \cellgray 57.5 & \cellgray 97.5 & \cellgray 97.5 & \cellgray 92.5 & \cellgray 30.0 & \cellgray 22.5 & \cellgray 97.5 & \cellgray 75.0  \\
& \ EN & \ 2.5 & \ 17.5 & \ 0.0 & \ 0.0 & \ 2.5 & \ 2.5 & \ 2.5 & \ 2.5 & \ 5.0  \\
& \ Tie & \ 62.5 & \ 25.0 & \ 2.5 & \ 2.5 & \ 5.0 & \ 67.5 & \ 75.0 & \ 0.0 & \ 20.0  \\
\midrule
\multirow{2}{*}{\textbf{GPT-3.5}}
& \cellgray CS & \cellgray 42.5 & \cellgray 50.0 & \cellgray 87.5 & \cellgray 82.5 & \cellgray 77.5 & \cellgray 57.5 & \cellgray 30.0 & \cellgray 72.5 & \cellgray 90.0  \\
& \ EN & \ 32.5 & \ 45.0 & \ 10.0 & \ 17.5 & \ 22.5 & \ 25.0 & \ 45.0 & \ 27.5 & \ 5.0  \\
& \ Tie & \ 25.0 & \ 5.0 & \ 2.5 & \ 0.0 & \ 0.0 & \ 17.5 & \ 25.0 & \ 0.0 & \ 5.0  \\
\midrule
\multirow{2}{*}{\textbf{Claude 3.5}}
& \cellgray CS & \cellgray 37.5 & \cellgray 55.0 & \cellgray 92.5 & \cellgray 100.0 & \cellgray 97.5 & \cellgray 27.5 & \cellgray 22.5 & \cellgray 95.0 & \cellgray 67.5  \\
& \ EN & \ 0.0 & \ 17.5 & \ 2.5 & \ 0.0 & \ 2.5 & \ 7.5 & \ 2.5 & \ 2.5 & \ 15.0  \\
& \ Tie & \ 62.5 & \ 27.5 & \ 5.0 & \ 0.0 & \ 0.0 & \ 65.0 & \ 75.0 & \ 2.5 & \ 17.5  \\
\midrule
\multirow{2}{*}{\textbf{Solar}}
& \cellgray CS & \cellgray 42.5 & \cellgray 82.5 & \cellgray 95.0 & \cellgray 100.0 & \cellgray 87.5 & \cellgray 40.0 & \cellgray 32.5 & \cellgray 97.5 & \cellgray 90.0  \\
& \ EN & \ 12.5 & \ 15.0 & \ 5.0 & \ 0.0 & \ 12.5 & \ 12.5 & \ 32.5 & \ 2.5 & \ 5.0  \\
& \ Tie & \ 45.0 & \ 2.5 & \ 0.0 & \ 0.0 & \ 0.0 & \ 47.5 & \ 35.0 & \ 0.0 & \ 5.0  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 70B}}
& \cellgray CS & \cellgray 35.0 & \cellgray 62.5 & \cellgray 67.5 & \cellgray 95.0 & \cellgray 95.0 & \cellgray 45.0 & \cellgray 42.5 & \cellgray 95.0 & \cellgray 77.5  \\
& \ EN & \ 32.5 & \ 25.0 & \ 30.0 & \ 5.0 & \ 5.0 & \ 15.0 & \ 22.5 & \ 5.0 & \ 17.5  \\
& \ Tie & \ 32.5 & \ 12.5 & \ 2.5 & \ 0.0 & \ 0.0 & \ 40.0 & \ 35.0 & \ 0.0 & \ 5.0  \\
\midrule
\multirow{2}{*}{\textbf{Llama3 8B}}
& \cellgray CS & \cellgray 50.0 & \cellgray 67.5 & \cellgray 82.5 & \cellgray 95.0 & \cellgray 77.5 & \cellgray 35.0 & \cellgray 45.0 & \cellgray 97.5 & \cellgray 85.0  \\
& \ EN & \ 35.0 & \ 32.5 & \ 17.5 & \ 5.0 & \ 22.5 & \ 47.5 & \ 37.5 & \ 2.5 & \ 12.5  \\
& \ Tie & \ 15.0 & \ 0.0 & \ 0.0 & \ 0.0 & \ 0.0 & \ 17.5 & \ 17.5 & \ 0.0 & \ 2.5  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 27B}}
& \cellgray CS & \cellgray 55.0 & \cellgray 72.5 & \cellgray 75.0 & \cellgray 100.0 & \cellgray 87.5 & \cellgray 52.5 & \cellgray 47.5 & \cellgray 97.5 & \cellgray 85.0  \\
& \ EN & \ 17.5 & \ 20.0 & \ 25.0 & \ 0.0 & \ 12.5 & \ 20.0 & \ 17.5 & \ 2.5 & \ 5.0  \\
& \ Tie & \ 27.5 & \ 7.5 & \ 0.0 & \ 0.0 & \ 0.0 & \ 27.5 & \ 35.0 & \ 0.0 & \ 10.0  \\
\midrule
\multirow{2}{*}{\textbf{Gemma2 9B}}
& \cellgray CS & \cellgray 65.0 & \cellgray 80.0 & \cellgray 82.5 & \cellgray 97.5 & \cellgray 90.0 & \cellgray 50.0 & \cellgray 50.0 & \cellgray 90.0 & \cellgray 82.5  \\
& \ EN & \ 7.5 & \ 12.5 & \ 15.0 & \ 2.5 & \ 10.0 & \ 27.5 & \ 20.0 & \ 7.5 & \ 10.0  \\
& \ Tie & \ 27.5 & \ 7.5 & \ 2.5 & \ 0.0 & \ 0.0 & \ 22.5 & \ 30.0 & \ 2.5 & \ 7.5  \\
\bottomrule






\end{tabular}
}

\caption{LLM Evaluation on Pairwise Comparison.}
\label{tab:llm_pair}

\end{table*}

==> tables/main_results_old.tex <==



\begin{table*}[!t]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{lc cccccccccc}
\toprule 
  Model & &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  Average \\
\midrule

\multirow{2}{*}{\textbf{GPT-4o}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{91.53} & \cellgray \textbf{\green{78.41}} & \cellgray \textbf{69.04} & \cellgray \textbf{\green{74.79}} & \cellgray \textbf{55.86} & \cellgray \textbf{\green{90.48}} & \cellgray \textbf{\green{95.12}} & \cellgray \textbf{63.7} & \cellgray \textbf{\green{85.14}} & \cellgray \textbf{78.23} \\
& EN & 89.83 & 75.00 & 66.19 & 61.97 & 52.64 & 84.52 & \textbf{\green{95.12}} & 60.4 & 74.32 & 73.33 \\
\midrule

\multirow{2}{*}{\textbf{GPT-3.5}} &
% \rowcolor{defaultcolor} 
\cellgray CS & \cellgray \textbf{71.19} & \cellgray 47.73 & \cellgray 44.48 & \cellgray 32.91 & \cellgray 35.40 & \cellgray \textbf{70.24} & \cellgray \textbf{80.49} & \cellgray 49.17 & \cellgray 57.21 & \cellgray \textbf{54.31} \\
& EN & \textbf{71.19} & \textbf{48.86} & \textbf{45.55} & \textbf{36.32} & \textbf{36.55} & 66.67 & 63.41 & \textbf{52.64} & \textbf{62.61} & 53.76 \\
\midrule

\multirow{2}{*}{\textbf{Claude 3.5}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{\green{93.22}} & \cellgray \textbf{72.16} & \cellgray \textbf{\green{72.95}} & \cellgray \textbf{73.08} & \cellgray \textbf{\green{62.53}} & \cellgray \textbf{86.90} & \cellgray \textbf{\green{95.12}} & \cellgray \textbf{\green{67.66}} & \cellgray \textbf{84.23} & \cellgray \textbf{78.65}
\\
& EN & 89.83 & 71.59 & 67.97 & 61.54 & 55.63 & 85.71 & 92.68 & 63.20 & 75.23 & 73.71 \\
\midrule

\multirow{2}{*}{\textbf{Solar}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{83.05} & \cellgray \textbf{55.11} & \cellgray \textbf{54.09} & \cellgray \textbf{63.46} & \cellgray \textbf{42.76} & \cellgray \textbf{80.95} & \cellgray \textbf{85.37} & \cellgray \textbf{54.29} & \cellgray \textbf{75.23} & \cellgray \textbf{66.03}
\\
& EN & 74.58 & 46.02 & 49.47 & 39.53 & \textbf{42.76} & 77.38 & 65.85 & 51.16 & 62.61 & 56.60 \\
\midrule

\multirow{2}{*}{\textbf{Llama3 70B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray 79.66 & \cellgray 51.70 & \cellgray \textbf{50.53} & \cellgray \textbf{49.36} & \cellgray 44.14 & \cellgray \textbf{80.95} & \cellgray \textbf{75.61} & \cellgray \textbf{57.43} & \cellgray 65.77 & \cellgray \textbf{61.68}
\\
& EN & \textbf{83.05} & \textbf{57.39} & \textbf{50.53} & 45.94 & \textbf{45.75} & 73.81 & 73.17 & 53.30 & \textbf{66.67} & 61.07 \\
\midrule

\multirow{2}{*}{\textbf{Llama3 8B}} &
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{69.49} & \cellgray \textbf{40.34} & \cellgray 36.30 & \cellgray 35.68 & \cellgray \textbf{35.63} & \cellgray \textbf{75.00} & \cellgray \textbf{73.17} & \cellgray 45.05 & \cellgray \textbf{54.05} & \cellgray \textbf{51.63}
\\
& EN & 64.41 & 39.77 & \textbf{37.72} & \textbf{37.39} & 32.64 & 67.86 & 63.41 & \textbf{45.21} & 53.6 & 49.11 \\
\midrule

\multirow{2}{*}{\textbf{Gemma2 27B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray 79.66 & \cellgray 46.02 & \cellgray \textbf{48.75} & \cellgray \textbf{41.03} & \cellgray \textbf{45.29} & \cellgray \textbf{77.38} & \cellgray \textbf{78.05} & \cellgray 54.79 & \cellgray \textbf{65.32} & \cellgray 59.59
\\
& EN & \textbf{84.75} & \textbf{53.41} & 48.40 & 40.6 & 41.84 & 72.62 & \textbf{78.05} & \textbf{54.95} & 63.96 & \textbf{59.84} \\
\midrule

\multirow{2}{*}{\textbf{Gemma2 9B}} & 
% \rowcolor{defaultcolor}
\cellgray CS & \cellgray \textbf{79.66} & \cellgray 42.05 & \cellgray 44.13 & \cellgray \textbf{40.17} & \cellgray 41.15 & \cellgray \textbf{73.81} & \cellgray \textbf{80.49} & \cellgray \textbf{53.30} & \cellgray \textbf{65.77} & \cellgray \textbf{57.84}
\\
& EN & 76.27 & \textbf{46.02} & \textbf{49.47} & 38.46 & \textbf{42.30} & 69.05 & 73.17 & 52.15 & 63.51 & 56.71 \\
\bottomrule
\end{tabular}
}

\caption{QA performances of multilingual LLMs on CS and English settings. \textbf{Bold} indicates higher score between CS and English on each model. \green{\textbf{Green}} indicates the highest score from each domain.}
\label{tab:plain_result}
\end{table*}



==> tables/og_kor_result_backup.tex <==

% 원본 한국어 데이터 결과

\begin{table*}[!ht]
\small
\centering
\resizebox{1\textwidth}{!}
{
\begin{tabular}{l cccccccccc}
\toprule 
  Model &
  \textbf{Economy} & \textbf{General} & \textbf{Geography} & \textbf{History} & \textbf{Law} & \textbf{Politics} & \textbf{Popular} & \textbf{Society} & \textbf{Tradition} & 
  \textbf{Total} \\
\midrule

\textbf{GPT-4o} & 94.92 & 76.70 & 75.09 & 76.50 & 58.62 & 89.29 & 97.56 & 67.00 & 85.59 & 80.14 \\
\midrule
\textbf{GPT-3.5} & 71.19 & 45.45 & 37.37 & 29.49 & 30.11 & 70.24 & 60.98 & 47.36 & 54.05 & 49.58 \\
\midrule
\textbf{Claude 3.5 Sonnet} & 89.83 & 71.59 & 80.78 & 76.28 & 66.67 & 89.29 & 95.12 & 71.45 & 87.39 & 80.93 \\
\midrule
\textbf{Solar} & 84.75 & 51.70 & 55.87 & 64.74 & 43.22 & 82.14 & 82.93 & 55.28 & 76.58 & 66.36 \\
\midrule
\textbf{Llama3 70B} & 86.44 & 52.27 & 53.38 & 51.50 & 41.84 & 77.38 & 82.93 & 59.41 & 68.92 & 63.79 \\
\midrule
\textbf{Llama3 8B} & 72.88 & 38.07 & 37.37 & 36.75 & 35.40 & 72.62 & 70.73 & 51.32 & 55.86 & 52.33 \\
\midrule
\textbf{Gemma2 27B} & 83.05 & 45.45 & 48.75 & 45.94 & 41.38 & 77.38 & 80.49 & 56.60 & 67.12 & 60.68 \\
\midrule
\textbf{Gemma2 9B} & 77.97 & 41.48 & 45.91 & 38.89 & 40.92 & 80.95 & 80.49 & 53.80 & 66.22 & 58.51 \\
\bottomrule

\end{tabular}
}

\caption{QA performances of LLMs on original Korean dataset.}
\label{tab:og_kor}
\end{table*}



==> tables/prompt_judge.tex <==
\begin{table*}[h]
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{Prompt for LLM-as-a-judge Evaluation} \\
    \midrule
You are a bilingual who is fluent in both Korean and English, and is knowledgeable about South Korea. You will be given a multiple choice question and a list of knowledge that are relevant to the question. The text are written in English-Korean code-switching, where matrix language is English and semantically important Korean words are embedded into English sentence. Your job is to follow the instructions and select one choice from [CHOICES].\\
\\
Instructions:\\
- Using given [KNOWLEDGE], explain concisely what and why you think is the answer. You can write in whichever language you can explain better, either Korean or English. Start this task with [EXPLANATION] tag.\\
- Choose your final choice from [CHOICES]. The answer is one of the [CHOICES], so do not say 'none of the above'. You must write a index number in parentheses, like (1). Start this task with [ANSWER] tag.\\
- Do not repeat input text in your response. Do not generate new question. Stick to input text that is given to you.\\

\\
I will give you an example for reference. \\
<<Example 1>>\\
{[QUESTION]}\\
Read the following question and choose the most appropriate answer. Who is the person who greatly defeated the soldiers of the 당나라 in the 안시성 싸움?\\
\\
{[CHOICES]}\\
(1) 양만춘\\
(2) 서희\\
(3) 김유신\\
(4) 강감찬\\
(5) 윤관\\
\\
{[KNOWLEDGE]}\\
1. 안시성 싸움 (Siege of Ansi): 안시성 싸움 (645 AD) was a famous military conflict between 고구려 and the 당 Dynasty. 고구려, under the leadership of 양만춘 (Yang Man-chun), successfully defended the 안시성 against the powerful 당 forces led by Emperor 태종.  \\
2. 양만춘 (Yang Man-chun): He was the general who commanded the defense of 안시성, playing a key role in defeating the 당나라 army.  \\
3. 서희 (Seo Hee): A 고려 diplomat famous for negotiating with the 거란 to avoid invasion, but not involved in the 안시성 싸움.  \\
4. 김유신 (Kim Yu-shin): A general from the 신라 Kingdom, instrumental in the unification of the 한반도, but not involved in this specific battle.  \\
5. 강감찬 (Gang Gam-chan): A 고려 military commander known for his victory over the 거란 in the 귀주대첩, unrelated to 안시성.  \\
6. 윤관 (Yun Gwan): A 고려 general famous for his campaigns against the Jurchen, unrelated to the 한반도.\\
\\
{[EXPLANATION]}\\
The question specifically asks about the 안시성 싸움 (Siege of Ansi) and who defeated the 당나라 soldiers in that battle. Based on historical facts, the leader who played a key role in defending 안시성 and defeating the 당나라 army was 양만춘 (Yang Man-chun).\\
\\
{[ANSWER]}\\
(1)\\
\\
Now solve this.\\
<<Example 2>>\\
{[QUESTION]}\\
\{question\}\\

{[CHOICES]}\\
\{choices\}\\
\\
{[KNOWLEDGE]}\\
\{knowledge\}\\

\\ \bottomrule
    \end{tabular}
    \caption{Prompt for Knowledge Leveraging task.}
    \label{tab:prompt_leveraging}
\end{table*}

